Composite Optimization with Error Feedback: the Dual Averaging Approach

Communication efficiency is a central challenge in distributed machine learning training, and message compression is a widely used solution. However, standard Error Feedback (EF) methods (Seide et al., 2014), though effective for smooth unconstrained optimization with compression (Karimireddy et al., 2019), fail in the broader and practically important setting of composite optimization, which captures, e.g., objectives consisting of a smooth loss combined with a non-smooth regularizer or constraints. The theoretical foundation and behavior of EF in the context of the general composite setting remain largely unexplored. In this work, we consider composite optimization with EF. We point out that the basic EF mechanism and its analysis no longer stand when a composite part is involved. We argue that this is because of a fundamental limitation in the method and its analysis technique. We propose a novel method that combines Dual Averaging with EControl (Gao et al., 2024), a state-of-the-art variant of the EF mechanism, and achieves for the first time a strong convergence analysis for composite optimization with error feedback. Along with our new algorithm, we also provide a new and novel analysis template for inexact dual averaging method, which might be of independent interest. We also provide experimental results to complement our theoretical findings.

==> appendices/analysis-econtrol-old.tex <==
\section{Old analysis}
%

In this section we present the missing proofs for the analysis of \Cref{alg:econtrol}.
Again, we remind the readers that for now we restrict ourselves to the setting where $a_t=1$ and $\gamma_t=\gamma$.
We first present the proof for \Cref{lem:e-descent-sum-in-h}.

\begin{restatable}{lemma}{EDescentSumInH}
\label{lem:e-descent-sum-in-h}
    We have
    \begin{equation}
        \label{eq:e-bar-descent-sum-in-h}
        \sum_{t=1}^{T}\bar E_t \leq \frac{1-\delta}{\eta^2}\sum_{t=0}^{T-1}H_t .
    \end{equation}
\end{restatable}

\begin{proof}
    We first give a descent for $ E_t$. By definition of $\ee_{t+1}^i$, we have:
    \[
        \ee_{t+1}^i \eqdef \hat \gg_t^i-\gg_t^i+\ee_t^i = \hat\gg_{t-1}^i+\Delta_t^i-\gg_t^i+\ee_t^i = \Delta_t^i-\delta_t^i + (1-\eta)\ee_t^i,
    \]
    where $\Delta_t\eqdef \avg{i}{n}\Delta_t^i$ and $\delta_t\eqdef \avg{i}{n}\delta_t^i$.
    Therefore:
    \begin{align*}
         \bar E_{t+1} &= \avg{i}{n}\norm{\Delta_t^i-\delta_t^i+(1-\eta)\ee_t^i}^2\\
        &\overset{(i)}{\leq} (1+\beta_1)(1-\eta)^2 \bar E_t + (1+\beta_1^{-1})\avg{i}{n}\norm{\Delta_t^i-\delta_t^i}^2\\
        &\overset{(ii)}{\leq} (1+\beta_1)(1-\eta)^2\bar E_t + (1+\beta_1^{-1})(1-\delta)\avg{i}{n}\norm{\delta_t^i}^2\\
        &=  (1+\beta_1)(1-\eta)^2\bar E_t + (1+\beta_1^{-1})(1-\delta)H_t,\,
    \end{align*}
    where in $(i)$ we used Young's inequality, and in $(ii)$ we used the definition of $\cC$. Now pick $\beta_1\eqdef \frac{\eta}{1-\eta}$, we get:
    \[
        \bar E_{t+1} \leq (1-\eta) \bar E_t + \frac{1-\delta}{\eta }H_t
    \]
    Therefore, by \Cref{lem:sum-lemma}, we have:
    \[
        \sum_{t=1}^{T}\bar E_t \leq \frac{1-\delta}{\eta^2}\sum_{t=0}^{T-1}H_t
    \]
\end{proof}

Next we give the proof of the \Cref{lem:h-descent-sum}.

\begin{restatable}{lemma}{HDescentSum}
    \label{lem:h-descent-sum}
    If $\eta\leq \frac{\delta'}{\sqrt{1+\delta'}+1}$ where $\delta'\eqdef \frac{\delta}{4-3\delta}$, then we have:
    \begin{equation}
        \label{eq:h-descent-sum}
        \sum_{t=0}^{T-1}\Eb{H_t} \leq \frac{32\eta^4}{\delta^2}\sum_{t=0}^{T-2}\Eb{\bar E_t} + \frac{32}{\delta^2 n}\sum_{t=0}^{T-2}\sum_{i=0}^{n}\EbNSq{\nabla f_i(\xx_{t+1})-\nabla f_i(\xx_t)} + \frac{64T\sigma^2}{\delta^2}
    \end{equation}
\end{restatable}
\begin{proof}
    We first note the following:
    \begin{align*}
        \delta_{t+1}^i &= \gg_{t+1}^i-\hat\gg_t^i -\eta\ee_{t+1}^i\\
        &= \gg_t^i - \hat\gg_t^i- \eta(\hat\gg_t^i-\gg_t^i+\ee_t^i) + \gg_{t+1}^i-\gg_t^i\\
        & = (1+\eta)(\gg_t^i-\hat\gg_t^i)  -\eta\ee_t^i + \gg_{t+1}^i-\gg_t^i\\
        & = (1+\eta)(\delta_t^i-\Delta_t^i+\eta\ee_t^i)-\eta\ee_t^i + \gg_{t+1}^i-\gg_t^i\\
        & = (1+\eta)(\delta_t^i-\Delta_t^i) +\eta^2\ee_t^i + \gg_{t+1}^i-\gg_t^i.
    \end{align*}
    Therefore, we have:
    \begin{align*}
        H_{t+1} & = \avg{i}{n}\norm{\delta_{t+1}^i}^2\\
        & = \avg{i}{n}\norm{(1+\eta)(\delta_t^i-\Delta_t^i) +\eta^2\ee_t^i + \gg_{t+1}^i-\gg_t^i}^2\\
        &\overset{(i)}{\leq} (1+\beta)(1+\eta)^2\avg{i}{n}\norm{\delta_t^i-\Delta_t^i}^2 + 4(1+\beta^{-1})\left(\eta^4\bar E_t +\avg{i}{n}\norm{\nabla f_i(\xx_{t+1})-\nabla f_i(\xx_t)}^2\right)\\
        &\quad +4(1+\beta^{-1})\left(\avg{i}{n}\norm{\gg_{t+1}^i-\nabla f_i(\xx_{t+1})}^2 + \avg{i}{n}\norm{\gg_{t}^i-\nabla f_i(\xx_{t})}^2\right)\\
        &\overset{(ii)}{\leq} (1+\beta)(1+\eta)^2(1-\delta)H_t + 2(1+\beta^{-1})\left(\eta^4\bar E_t + \avg{i}{n}\norm{\nabla f_i(\xx_{t+1})-\nabla f_i(\xx_t)}^2\right)\\
        &\quad +4(1+\beta^{-1})\left(\avg{i}{n}\norm{\gg_{t+1}^i-\nabla f_i(\xx_{t+1})}^2 + \avg{i}{n}\norm{\gg_{t}^i-\nabla f_i(\xx_{t})}^2\right),\,
    \end{align*}
    where in $(i)$ we used Young's inequality with $\beta>0$, and in $(ii)$ we used the definition of $H_t$ and the fact that $\cC$ is a compression operator.

    Now we pick $\beta = \frac{\delta}{4(1-\delta)}$. Therefore, $(1+\beta)(1+\eta)^2(1-\delta)=(1-\frac{3\delta}{4})(1+\eta)^2$. We pick $\eta$ small enough such that $(1-\frac{3\delta}{4})(1+\eta)^2\leq 1-\frac{\delta}{2}$. It suffices to have $\eta\leq \frac{\delta'}{\sqrt{1+\delta'}+1}$ where $\delta'\eqdef \frac{\delta}{4-3\delta}$. 
    %
    Therefore, we have:
    \begin{align*}
        H_{t+1} &\leq (1-\frac{\delta}{2})H_t + \frac{(16-12\delta)\eta^4}{\delta}\bar E_t + \frac{16-12\delta}{\delta n}\sum_{i=0}^{n}\norm{\nabla f_i(\xx_{t+1})-\nabla f_i(\xx_t)}^2\\
        &\quad +\frac{16-12\delta}{\delta}\left(\avg{i}{n}\norm{\gg_{t+1}^i-\nabla f_i(\xx_{t+1})}^2 + \avg{i}{n}\norm{\gg_{t}^i-\nabla f_i(\xx_{t})}^2\right)
    \end{align*}
    Taking expectation, we get:
    \begin{align*}
        \EEb{\xi_{t+1},\xi_t}{H_{t+1}\vert \xi_0,\dots,\xi_{t-1}} &\leq (1-\frac{\delta}{2})\EEb{\xi_{t}}{H_{t}\vert \xi_0,\dots,\xi_{t-1}} + \frac{(16-12\delta)\eta^4}{\delta}\EEb{\xi_{t}}{\bar E_{t}\vert \xi_0,\dots,\xi_{t-1}} \\
        &\quad + \frac{16-12\delta}{\delta n}\sum_{i=0}^{n}\EEb{\xi_{t}}{\norm{\nabla f_i(\xx_{t+1})-\nabla f_i(\xx_t)}^2\vert \xi_0,\dots,\xi_{t-1}}\\
        &\quad  +\frac{(32-24\delta)\sigma^2}{\delta}
    \end{align*}

    Due to the initialization of $\gg_0^i=\nabla f_i(\xx_0)$ and $\ee_0^i=\0$, we have $H_0=0$. Now we apply \Cref{lem:sum-lemma} and law of total expectation to get:
    \[
        \sum_{t=0}^{T-1}\EEb{\xi_0,\dots,\xi_t}{H_t} \leq \frac{32\eta^4}{\delta^2}\sum_{t=0}^{T-2}\EEb{\xi_0,\dots,\xi_t}{\bar E_t} + \frac{32}{\delta^2 n}\sum_{t=0}^{T-2}\sum_{i=0}^{n}\EEb{\xi_0,\dots,\xi_t}{\norm{\nabla f_i(\xx_{t+1})-\nabla f_i(\xx_t)}^2} + \frac{64\eta^4T\sigma^2}{\delta^2}
    \]
\end{proof}

Next we give an upper bound on the distance between $\hat \gg_t$ and $\nabla f(\xx_t)$:

\begin{restatable}{lemma}{DistGhatG}
    \label{lem:dist-ghat-g}
    Given \Cref{assumption:bounded_variance}, we have:
    \begin{equation}
        \label{eq:dist-ghat-g}
        \EbNSq{\hat \gg_t-\nabla f(\xx_t)} \leq 3(1-\delta)\Eb{H_t} + 3\eta^2\Eb{\bar E_t} + \frac{3\sigma^2}{n}
    \end{equation}
\end{restatable}

\begin{proof}
    \begin{align*}
        \norm{\hat \gg_t-\nabla f(\xx_t)}^2 &= \norm{\Delta_t-(\gg_t-\hat\gg_{t-1}-\eta\ee_t) -\eta\ee_t+\gg_t-\nabla f(\xx_t)}^2 \\
        &\leq 3\norm{\Delta_t-\delta_t}^2 + 3\eta^2\norm{\ee_t}^2+ 3\norm{\gg_t-\nabla f(\xx_t)}^2\\
        &\leq 3\avg{i}{n}\norm{\Delta_t^i-\delta_t^i}^2 + 3\eta^2\bar E_t+ 3\norm{\gg_t-\nabla f(\xx_t)}^2\\
        &\leq 3(1-\delta)H_t+3\eta^2\bar E_t + 3\norm{\gg_t-\nabla f(\xx_t)}^2
    \end{align*}
    Taking expectation, we get the desired result.
\end{proof}

Next we give the upper bound on the distance between consecutive iterates:
\begin{restatable}{lemma}{XDistanceEControlDA}
    \label{lem:x-distance-econtrol-da}
    Given \Cref{assumption:smoothness}, we have:
    \begin{equation}
        \label{eq:x-distance-econtrol-da}
        \sum_{t=0}^{T-1}\frac{\gamma- L}{2}\EbNSq{\xx_{t+1}-\xx_t}\leq \Eb{F(\xx_0)-F(\xx_T)} + \frac{3}{2\gamma}\sum_{t=0}^{T-1}\left((1-\delta) \Eb{H_t} +\eta^2\Eb{\bar E_t}\right) + \frac{3T\sigma^2}{2\gamma n}
    \end{equation}
\end{restatable}

\begin{proof}
    We take \Cref{eq:x-distance-da} and set $a_t=1$ and $\gamma_t=\gamma$ for all $t$. Note that $\beta_t$'s are constants so that $\sum_{t=0}^{T-1}(\beta_t\rho_t^2-\beta_t\rho_{t+1}^2)=0$. We have:
    \[
        \sum_{t=0}^{T-1}\left(\frac{2\gamma-L}{2}\norm{\xx_{t+1}-\xx_t}^2 + \inp{\hat \gg_t-\nabla f(\xx_t)}{\xx_{t+1}-\xx_t}\right) \leq F(\xx_0)-F(\xx_{T})
    \]
    Now we apply Young's inequality and get:
    \begin{align*}
        \sum_{t=0}^{T-1}\frac{\gamma-L}{2}\EbNSq{\xx_{t+1}-\xx_t} &\leq \Eb{F(\xx_0)-F(\xx_{T})} + \frac{1}{2\gamma}\sum_{t=0}^{T-1}\EbNSq{\hat \gg_t-\nabla f(\xx_t)}\\
        &\leq \Eb{F(\xx_0)-F(\xx_{T})} + \frac{1}{2\gamma}\sum_{t=0}^{T-1}\left(3(1-\delta)\Eb{H_t} + 3\eta^2\Eb{\bar E_t} + \frac{3\sigma^2}{n}\right)
    \end{align*}
\end{proof}


Now we give an upper bound on the sum of error terms $\bar E_t$ and prove \Cref{lem:e-sum-da}:

\begin{restatable}{lemma}{ESumDA}
    \label{lem:e-sum-da}
    Given \Cref{assumption:smoothness,assumption:ell-smoothness}, setting $\eta\eqdef\frac{\delta}{12}$ and assuming that $\gamma\geq \frac{28\ell}{\delta}$, we have:
    \begin{equation}
        \label{eq:e-sum-da}
        \sum_{t=1}^{T}\Eb{\bar E_t }\leq  \frac{2^{15}\ell^2}{\delta^4\gamma}F_0 + \frac{2^{14}T\sigma^2}{\delta^4},\,
    \end{equation}
    where $F_0\eqdef F(\xx_0)-F^\star$.
\end{restatable}

\begin{proof}
    By \Cref{assumption:smoothness,assumption:ell-smoothness} and \Cref{lem:h-descent-sum}, we have:
    \begin{align*}
        \sum_{t=0}^{T-1}\Eb{H_t} &\leq \frac{32\eta^4}{\delta^2}\sum_{t=0}^{T-2}\Eb{\bar E_t} + \frac{32}{\delta^2 n}\sum_{t=0}^{T-2}\sum_{i=0}^{n}\EbNSq{\nabla f_i(\xx_{t+1})-\nabla f_i(\xx_t)} + \frac{64T\sigma^2}{\delta^2}\\
        &\leq \frac{32\eta^4}{\delta^2}\sum_{t=0}^{T-2}\Eb{\bar E_t} + \frac{32\ell^2}{\delta^2}\sum_{t=0}^{T-2}\EbNSq{\xx_{t+1}-\xx_t} + \frac{64T\sigma^2}{\delta^2}
    \end{align*}
    Now we apply \Cref{eq:x-distance-econtrol-da}, and get:
    \begin{align*}
        \sum_{t=0}^{T-1}\Eb{H_t} &\leq \frac{32\eta^4}{\delta^2}\sum_{t=0}^{T-2}\Eb{\bar E_t} + \frac{32\ell^2}{\delta^2(\gamma -L) }\left(2\Eb{F(\xx_0)-F(\xx_T)} + \frac{3}{\gamma}\sum_{t=0}^{T-1}\left((1-\delta) \Eb{H_t} +3\eta^2\Eb{\bar E_t}\right)\right)\\
        &\quad + \frac{64T\sigma^2}{\delta^2} + \frac{96\ell^2T\sigma^2}{\gamma(\gamma- L)n}\\
            &= \frac{96\ell^2(1-\delta)}{\delta^2 \gamma(\gamma - L)}\sum_{t=0}^{T-2}\Eb{H_t}+ \left(\frac{32\eta^4}{\delta^2}+ \frac{96\ell^2\eta^2}{\delta^2\gamma(\gamma- L)}\right)\sum_{t=0}^{T-2}  \Eb{\bar E_t} + \frac{64\ell^2}{\delta^2 (\gamma -L)}\Eb{F(\xx_0)-F(\xx_{T-1})}\\
            &\quad + \frac{64T\sigma^2}{\delta^2} + \frac{96\ell^2T\sigma^2}{\gamma(\gamma- L)n}
    \end{align*}
    Now we apply \Cref{lem:e-descent-sum-in-h} and get:
    \begin{align*}
        \sum_{t=0}^{T-1}\Eb{H_t} &\leq \frac{96\ell^2(1-\delta)}{\delta^2 \gamma(\gamma - L)}\sum_{t=0}^{T-2}\Eb{H_t}+ \left(\frac{32\eta^2}{\delta^2}+ \frac{96\ell^2}{\delta^2\gamma(\gamma- L)}\right)\sum_{t=0}^{T-1}  \Eb{H_t} + \frac{64\ell^2}{\delta^2 \gamma(\gamma -L)}\Eb{F(\xx_0)-F(\xx_{T-1})}\\
            &\quad + \frac{64T\sigma^2}{\delta^2} + \frac{96\ell^2T\sigma^2}{\gamma(\gamma- L)n}
    \end{align*}
    Now let's assume that $\gamma \geq 2L$, then we have:
    \begin{align*}
        \sum_{t=0}^{T-1}\Eb{H_t} &\leq \frac{192\ell^2}{\delta^2\gamma^2}\sum_{t=0}^{T-2}\Eb{H_t}+ \left(\frac{32\eta^2}{\delta^2}+ \frac{192\ell^2}{\delta^2\gamma^2}\right)\sum_{t=0}^{T-1} \Eb{H_t} + \frac{128\ell^2}{\delta^2\gamma}\Eb{F(\xx_0)-F(\xx_{T-1})}\\
        &\quad + \frac{64T\sigma^2}{\delta^2} + \frac{192\ell^2T\sigma^2}{\gamma^2n}
    \end{align*}
    We also pick $\eta=\frac{\delta}{12}$, which satisfies the assumption of \Cref{lem:h-descent-sum}. And we also require $\gamma \geq \frac{28\ell}{\delta}$, implying that $\frac{384\ell^2}{\delta^2\gamma^2}\leq \frac{1}{2}$. Rearranging, we have:
    \[
        \sum_{t=0}^{T-1} \Eb{H_t}\leq \frac{178\ell^2}{\delta^2\gamma}\Eb{F(\xx_0)-F(\xx_{T-1})} + \frac{90T\sigma^2}{\delta^2}
    \]
    Now we apply \Cref{lem:e-descent-sum-in-h} again and get:
    \[
        \sum_{t=1}^{T}\Eb{\bar E_t }\leq \frac{2^{15}\ell^2}{\delta^4\gamma}\Eb{F(\xx_0)-F(\xx_{T-1})} + \frac{2^{14}T\sigma^2}{\delta^4}
    \]

\end{proof}

Finally, we prove \Cref{thm:econtrol-da}:

\EControlDA*

\begin{proof}

    For simplicity of notation, let's write $F_t\eqdef F(\wtilde\xx_t)-F(\xx^\star)$.

    By \Cref{lem:e-sum-da} and \Cref{thm:main-descent-xx-virtual-da}, we have, when $\gamma \geq \frac{28\ell}{\delta}$:

    \begin{align*}
        \frac{1}{T} \sum_{t=0}^{T-1}\Eb{F_{t+1}} &\leq   \frac{\gamma R_0^2}{2T}+\frac{ L}{\gamma^2T}\sum_{t=0}^{T-1}\EbNSq{\ee_t} + \frac{\sigma^2}{\gamma n}\\
            &\leq  \frac{\gamma R_0^2}{2T}+\frac{2^{15}\ell^2L}{\gamma^3\delta^4T}F_0 + \frac{2^{14}L\sigma^2}{\gamma^2\delta^4} + \frac{\sigma^2}{\gamma n},\,
    \end{align*}
    where we write $F_t\eqdef \Eb{F(\wtilde\xx_t) - F(\xx^\star)}$.

    Now we choose $\gamma=\max\left\{\frac{28\ell}{\delta}, \frac{14L^{\nicefrac{1}{4}}\ell^{\nicefrac{1}{2}}F_0^{\nicefrac{1}{4}}}{\delta R_0^{\nicefrac{1}{2}}}, \sqrt{\frac{2T\sigma^2}{nR_0^2}}, \frac{32T^{\nicefrac{1}{3}}L^{\nicefrac{1}{3}}\sigma^{\nicefrac{2}{3}}}{R_0^{\nicefrac{2}{3}}\delta^{\nicefrac{4}{3}}} \right\}$, we have:
    \[
        \frac{1}{T}\sum_{t=1}^{T}\Eb{F_t} \leq \frac{14\ell R_0^2}{\delta T} + \frac{7L^{\nicefrac{1}{4}}\ell^{\nicefrac{1}{2}}F_0^{\nicefrac{1}{4}}R_0^{\nicefrac{3}{2}}}{\delta T} + \sqrt{\frac{R_0^2\sigma^2}{2nT}} + \frac{16R_0^{\nicefrac{4}{3}}L^{\nicefrac{1}{3}}\sigma^{\nicefrac{2}{3}}}{T^{\nicefrac{2}{3}}\delta^{\nicefrac{4}{3}}}
    \]

    Therefore, after:
    \[
        T = 16\left(\frac{8R_0^2\sigma^2}{n\varepsilon^2}+ \frac{512R_0^2\sqrt{L}\sigma}{\delta^2\varepsilon^{\nicefrac{3}{2}}} + \frac{56\ell R_0^2}{\delta \varepsilon} + \frac{28L^{\nicefrac{1}{4}}\ell^{\nicefrac{1}{2}}F_0^{\nicefrac{1}{4}}R_0^{\nicefrac{3}{2}}}{\delta \varepsilon}\right),\,
    \]
    iterations of \Cref{alg:econtrol-da}, we have:
    \[
        \frac{1}{T}\sum_{t=1}^{T}\Eb{F_t} \leq \varepsilon.
    \]

    Note that this already gives us the desirable convergence rate. We can further simplify the above rates and remove the dependence on $F_0$ by taking one additional stochastic gradient step initially to get $\xx_0'$. By \Cref{lem:gradient-step-upper-bound}, we have $\Eb{F(\xx_0')-F^\star}\leq LR_0^2+\frac{R_0\sigma}{\sqrt{2}}$ and $R_0'\eqdef \EbNSq{\xx_0'-\xx^\star}\leq \sqrt{2}R_0$. Therefore if we start our algorithm at $\xx_0'$, then we have:
    \[
        \frac{1}{T} \sum_{t=0}^{T-1}\Eb{F_{t+1}} \leq  \frac{\gamma R_0^2}{2T}+\frac{2^{15}\ell^2L^2R_0^2}{\gamma^3\delta^4T}+\frac{2^{15}\ell^2LR_0\sigma}{\gamma^3\delta^4T} + \frac{2^{14}L\sigma^2}{\gamma^2\delta^4} + \frac{\sigma^2}{\gamma n}
    \]
    Now we pick:
    \[
        \gamma=\max\left\{\frac{28\ell}{\delta}, \frac{16\ell^{\nicefrac{1}{2}}L^{\nicefrac{1}{2}}}{\delta}, \frac{16\ell^{\nicefrac{1}{2}}L^{\nicefrac{1}{4}}\sigma^{\nicefrac{1}{4}}}{\delta R_0^{\nicefrac{1}{4}}}, \sqrt{\frac{2T\sigma^2}{nR_0^2}}, \frac{32T^{\nicefrac{1}{3}}L^{\nicefrac{1}{3}}\sigma^{\nicefrac{2}{3}}}{R_0^{\nicefrac{2}{3}}\delta^{\nicefrac{4}{3}}} \right\},\,
    \]
    and we have:
    \begin{align*}
        \frac{1}{T}\sum_{t=1}^{T}\Eb{F_t} &\leq \frac{14\ell R_0^2}{\delta T} + \frac{8(\ell L)^{\nicefrac{1}{2}}R_0^2}{\delta T} + \frac{8\ell^{\nicefrac{1}{2}}L^{\nicefrac{1}{4}}R_0^{\nicefrac{7}{4}}\sigma^{\nicefrac{1}{4}}}{\delta T} + \sqrt{\frac{R_0^2\sigma^2}{2nT}} + \frac{16R_0^{\nicefrac{4}{3}}L^{\nicefrac{1}{3}}\sigma^{\nicefrac{2}{3}}}{T^{\nicefrac{2}{3}}\delta^{\nicefrac{4}{3}}}\\
        &\leq \frac{22\ell R_0^2}{\delta T} + \frac{8\ell^{\nicefrac{1}{2}}L^{\nicefrac{1}{4}}R_0^{\nicefrac{7}{4}}\sigma^{\nicefrac{1}{4}}}{\delta T} + \sqrt{\frac{R_0^2\sigma^2}{2nT}} + \frac{16R_0^{\nicefrac{4}{3}}L^{\nicefrac{1}{3}}\sigma^{\nicefrac{2}{3}}}{T^{\nicefrac{2}{3}}\delta^{\nicefrac{4}{3}}}
    \end{align*}

    Therefore, we need only:
    \[
        T = 16\left(\frac{22R_0^2\sigma^2}{n\varepsilon^2}+ \frac{512R_0^2\sqrt{L}\sigma}{\delta^2\varepsilon^{\nicefrac{3}{2}}} + \frac{56\ell R_0^2}{\delta \varepsilon} + \frac{8\ell^{\nicefrac{1}{2}}L^{\nicefrac{1}{4}}R_0^{\nicefrac{7}{4}}\sigma^{\nicefrac{1}{4}}}{\delta \varepsilon}\right),\,
    \]
    iterations. Moreover, let's discuss the last term more carefully:

    If $LR_0^2\geq R_0\sigma$: in this case, the last term is upper bounded by $\frac{8\ell R_0^2}{\delta \varepsilon}$.

    On the other hand, if $LR_0^2\leq R_0\sigma$: we have that $F_0\leq 2R_0\sigma$. In particular, in this case, we can assume that $\varepsilon \leq 2R_0\sigma$, otherwise we don't need to take any step. In this case, 
    \[
        \frac{8\ell^{\nicefrac{1}{2}}L^{\nicefrac{1}{4}}R_0^{\nicefrac{7}{4}}\sigma^{\nicefrac{1}{4}}}{\delta \varepsilon}=\frac{(\ell R_0^2)^{\nicefrac{1}{2}}(L R_0^2)^{\nicefrac{1}{4}}(R_0\sigma)^{\nicefrac{1}{4}}\varepsilon^{\nicefrac{1}{2}}}{\delta \varepsilon^{\nicefrac{3}{2}}}\leq \frac{\sqrt{2}R_0^2\sqrt{\ell}\sigma}{\delta \varepsilon^{\nicefrac{3}{2}}}
    \]
    Therefore, it takes at most:
    \[
        T = 16\left(\frac{22R_0^2\sigma^2}{n\varepsilon^2}+ \frac{514R_0^2\sqrt{\ell}\sigma}{\delta^2\varepsilon^{\nicefrac{3}{2}}} + \frac{64\ell R_0^2}{\delta \varepsilon} \right)
    \]
    iterations of \Cref{alg:econtrol-da} to get:
    \[
        \frac{1}{T}\sum_{t=1}^{T}\Eb{F_t} \leq \varepsilon.
    \]

        

\end{proof}

==> appendices/prox-real-iterates.tex <==
\section{Analysis of the Proximal \algname{EControl}}
\label{sec:analysis-proximal-econtrol}


==> dual_avg/da_new.tex <==
In this section we present a general recipe for analyzing dual averaging methods with inexact gradients. We do not restrict ourselves to the case of communication compression, or indeed, any particular source of inexactness.  The inexactness might come from compression of the gradients, or from the point at which the gradients are queried. Interestingly, the latter case is also crucial for our analysis of the communicaiton compression setting and provides a clearer perspective on the virtual iterates framework widely used in the literature.


\begin{algorithm}[tb]
    \caption{Inexact Dual Averaging}
    \label{alg:da}
    \begin{algorithmic}[1]
        \State \textbf{Input:} $\yy_0$ and stepsizes $\{a_t\}_{t=0,1,\dots,\infty}$.
        \For{$t = 0,1,\dots$}
            \State Obtain $\hat \gg_t\approx \gg_t\eqdef \nabla f(\yy_t)$ \Comment{e.g. $\hat\gg_t = \nabla f(\yy_t')$ for some $\yy_t'\approx \yy_t$; } 
            \State ~ \Comment{or $\hat\gg_t = \cT(\nabla f(\yy_t)\vert \{\yy_s\}_{s\in[t-1]})$ for some transformation $\cT$}
            \State $\yy_{t+1} =\argmin_{\yy}\left[ 
                \Phi_t(\yy) \eqdef
                \sum_{s=0}^{t} a_s(f(\yy_s)+\inp{\hat{\gg}_s}{\yy-\yy_s}+\psi(\yy))
                +
                \frac{1}{2} \norm{\yy - \yy_0}^2
            \right]$
        \hfill
        \EndFor
    \end{algorithmic}
\end{algorithm}

\begin{theorem}
    \label{thm:da-inexact}
    Given \Cref{assumption:convexity,assumption:smoothness},
\end{theorem}
\begin{proof}
    By the definition of $\Phi_t$, we have for any $\yy\in {\rm dom}(\psi)$:
    \[
        \Phi_t(\yy) \geq \Phi_t(\yy_t) + \frac{1}{2}\norm{\yy-\yy_t}^2
    \]
    We also have:
    \begin{align*}
        \Phi_t(\yy) &= \sum_{s=0}^{t-1} a_s(f(\yy_s)+\inp{\hat\gg_s}{\yy-\yy_s}+\psi(\yy)) + \frac{1}{2} \norm{\yy - \yy_0}^2\\
        &= \sum_{s=0}^{t-1} a_s(f(\yy_s)+\inp{\nabla f(\yy_s)}{\yy-\yy_s}+\psi(\yy)) + \sum_{s=0}^{t-1}a_s\inp{\hat\gg_s-\nabla f(\yy_s)}{\yy-\yy_s} + \frac{1}{2} \norm{\yy - \yy_0}^2\\
        &\overset{(i)}{\leq }\sum_{s=0}^{t-1}a_sF(\yy)+ \sum_{s=0}^{t-1}a_s\inp{\hat\gg_s-\nabla f(\yy_s)}{\yy-\yy_s} + \frac{1}{2} \norm{\yy - \yy_0}^2,\,
    \end{align*}
    where in $(i)$ we used the convexity of $f$. Now by the definition of $\yy_{t+1}$:
    \begin{align*}
        \Phi_{t+1}(\yy_{t+1}) &= \Phi_t(\yy_{t+1}) + a_t(f(\yy_t) + \inp{\hat\gg_t}{\yy_{t+1}-\yy_t} + \psi(\yy_{t+1}))\\
            &\overset{(ii)}{\geq} \Phi_t(\yy_t) + \frac{1}{2}\norm{\yy_{t+1}-\yy_t}^2 + a_s(f(\yy_t) + \inp{\hat\gg_t}{\yy_{t+1}-\yy_t} + \psi(\yy_{t+1}))\\
            &= \Phi_t(\yy_t) + \frac{1}{2}\norm{\yy_{t+1}-\yy_t}^2 + a_t(f(\yy_t) + \inp{\nabla f(\yy_t)}{\yy_{t+1}-\yy_t} + \psi(\yy_{t+1})) + a_t\inp{\hat\gg_t-\nabla f(\yy_t)}{\yy_{t+1}-\yy_t}\\
            &\overset{(iii)}{\geq} \Phi_t(\yy_t) + \frac{1-a_tL}{2}\norm{\yy_{t+1}-\yy_t}^2 + a_tF(\yy_{t+1})  + a_t\inp{\hat\gg_t-\nabla f(\yy_t)}{\yy_{t+1}-\yy_t},\,
    \end{align*}
    where in $(ii)$ we used the 1-strong convexity of $\Phi_t$ and in $(iii)$ we used \Cref{assumption:smoothness}.

    Now rearranging and summing from $t=0$ to $T-1$, we get:
    \begin{align*}
        \sum_{t=0}^{T-1}a_tF(\yy_{t+1}) + \frac{1-a_tL}{2}\norm{\yy_{t+1}-\yy_t}^2 &\leq \Phi_{T}(\yy_T)  - \sum_{t=0}^{T-1}a_t\inp{\hat\gg_t-\nabla f(\yy_t)}{\yy_{t+1}-\yy_t}\\
        &\leq \Phi_T(\yy) - \frac{1}{2}\norm{\yy-\yy_T}^2 - \sum_{t=0}^{T-1}a_t\inp{\hat\gg_t-\nabla f(\yy_t)}{\yy_{t+1}-\yy_t}\\
        &\leq \sum_{t=0}^{T-1}a_tF(\yy)+ \sum_{t=0}^{T-1}a_t\inp{\hat\gg_t-\nabla f(\yy_t)}{\yy-\yy_t} + \frac{1}{2} \norm{\yy - \yy_0}^2\\
        &\quad - \frac{1}{2}\norm{\yy-\yy_T}^2 - \sum_{t=0}^{T-1}a_t\inp{\hat\gg_t-\nabla f(\yy_t)}{\yy_{t+1}-\yy_t}
    \end{align*}
    Rearranging, we get:
    \[
        \sum_{t=0}^{T-1}[a_t(F(\yy_{t+1})-F(\yy)) + \frac{1-a_tL}{2}\norm{\yy_{t+1}-\yy_t}^2] \leq \frac{1}{2}(\norm{\yy-\yy_0}^2-\norm{\yy-\yy_T}^2)+ \sum_{t=0}^{T-1} a_t\inp{\hat\gg_t-\nabla f(\yy_t)}{\yy-\yy_{t+1}} 
    \]
\end{proof}
